Do Children Texts Hold The Key To Commonsense Knowledge?

Compiling comprehensive repositories of commonsense knowledge is a long-standing problem in AI. Many concerns revolve around the issue of reporting bias, i.e., that frequency in text sources is not a good proxy for relevance or truth. This paper explores whether children's texts hold the key to commonsense knowledge compilation, based on the hypothesis that such content makes fewer assumptions on the reader's knowledge, and therefore spells out commonsense more explicitly. An analysis with several corpora shows that children's texts indeed contain much more, and more typical commonsense assertions. Moreover, experiments show that this advantage can be leveraged in popular language-model-based commonsense knowledge extraction settings, where task-unspecific fine-tuning on small amounts of children texts (childBERT) already yields significant improvements. This provides a refreshing perspective different from the common trend of deriving progress from ever larger models and corpora.

==> parts/summarization.tex <==
\section{Text Summarization}

Not enough difference with automatic metrics and too hard for manual annotation.

TLDR?
Other texts to summarize. - something less entity-centric (as news corpora are)

\begin{table*}[ht]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        Corpus & ROUGE-1 & ROUGE-2 & ROUGE-L & Mean summary length\\
        \hline
        None & 44.15 & 21.29 & 31.08 & 75.63 \\
        InfantBooks & 44.01 & 21.31 & 31.14 & 72.95 \\
        C4 easy & 43.1 & 20.8 & 30.8 & 67.2 \\
        
        \hline
    \end{tabular}
    \caption{Results of Text Summarization}
    \label{tab:summarization}
\end{table*}

==> parts/typicality_old.tex <==
\paragraph{CSK Typicality.}
Human associations and CSK resources contain a mix of salient but atypical assertions (\textit{lion attacks human}), and typical but basic assertions (\textit{lion drinks water}). To evaluate whether children texts can help to extract more typical assertions, we use PTLM prompting.

We used the BERT-large model\footnote{\href{https://huggingface.co/bert-large-uncased}{https://huggingface.co/bert-large-uncased}}, and fine-tuned it on each of the four corpora, up to a maximum of 48 hours (using one NVIDIA Quadro RTX 8000). We used a learning rate of $1e^{-5}$.

We then used 1,600 CSK triples from Quasimodo \cite{quasimodo}, human-rated as \textit{very typical} (score [1,2[), or \textit{typical} (score [2,3[), or \textit{plausible} (score [3,4[) as targets. For each of these triples, we masked the objects, and used the fine-tuned BERT model to predict token likelihoods for the mask. 


%We used the same pretrained LM for all the approaches, a large BERT model pretrained on the English Wikipedia and BookCorpus. Then, we fine-tune on each corpus. We limited this step to 48 hours.  Doing the pretraining on InfantBooks takes between one and two minutes on a \textit{NVIDIA Quadro RTX 8000}. Doing it on CBT takes around 20 minutes on the same machine. For InfantBooks and CBT, we vary the number of epoch between 1 and 10 with a learning rate of $1e^{-5}$. For C4 corpora, we used a learning rate of $1e^{-5}$ when training a few training steps. Otherwise, we use a learning rate of $1e^{-7}$. Finally, we report the Mean Reciprocal Rank (MRR), the precision at 1 (P@1), and the precision at 10 (P@10).

 
%To test if a language model prefers typical statements, we ask MTurks to annotate sentences coming from Quasimodo by typicality. We asked them to give a score between 1 and 5, 1 meaning that a statement can always be observed while 5 means that the fact is never observed. In total, we annotated 1,600 sentences with two annotators per statement. Then, we hide the object in each statement and, using an LM trained from BERT like in Section~\ref{sec:lama}, we compute the rank of the correct hidden word. We report the median ranks in Table~\ref{tab:typicality}


\begin{table}[ht]
     \centering
     \small
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
         BERT-finetuning & Very typical & Typical & Plausible \\
         \hline
         None & 0.361 & 0.200 & 0.153 \\
         InfantBooks & \textbf{0.364} & 0.198 & 0.152\\
         CBT & \textbf{0.364} & \textbf{0.205} & 0.148\\
         C4-easy & 0.326 & 0.204 & \textbf{0.156}\\
%         C4-hard & 13 & 89 & 155 & 246 & 490 \\
         C4 & 0.312 & 0.195 & 0.155\\
         \hline
    \end{tabular}
    \caption{Mean reciprocal ranks of typical statements.}
    \label{tab:typicality}
\end{table}

In Table \ref{tab:typicality} we report the median reciprocal rank for each group. InfantBooks and CBT have a significant advantage in predicting very typical and typical statements.




%InfantBook beats the other approaches for the most typical statements. CBT also has good results, showing that even books for older children can be helpful to capture typical commonsense. Surprisingly, the models derived from C4 give worst results than a standard BERT for the most typical statements. Otherwise, it generates statements with a lower rank. The results for non-typical statements are hard to interpret: We would like to have a high rank to avoid having non-typical facts, but the original statements are correct (and extracted from actual texts). So, the rank should not be too high either.
